Maneuvering, Multi-Target Tracking using Particle Filters

In this work, we develop tracking and estimation techniques relevant to underwater targets. Particularly, we explore particle filtering techniques for target tracking. It is a numerical approximation method for implementing a recursive Bayesian estimation procedure. It does not require the assumptions of linearity and Guassianity like the traditional Kalman filter based techniques and is capable of handling non-Gaussian noise distributions and non-linearities in the measurements as well as target dynamics. The performance of particle filters is verified using simulations and compared with Extended Kalman Filter. Particle filters can track multi-targets and highly maneuvering targets. However, it has higher computational load. The efficient use of particle filters for multi-target tracking using Independent Partition Particle Filter (IPPF) and tracking highly maneuvering targets using Multiple Model Particle Filter(MMPF) are also explored in this work. These techniques require only smaller number of particles and help in reducing the computational cost. Data association problem exists in multi-target tracking due to lack of information at the observer about the proper association between the targets and the received measurements. The problem becomes more involved when the targets move much closer and there are clutter and missed target detections at the observer. Monte Carlo Joint Probabilistic Data Association Filter (MCJPDAF) efficiently solves data association for the mentioned situation. Due to the inability of the standard MCJPDAF to track highly maneuvering targets, Monte Carlo Multiple Model Joint Probabilistic Data Association Filter (MC-MMJPDAF) which combines the technique of Multiple Model Particle Filter(MMPF) in the framework of MC-JPDAF has been proposed. The simulation results shows the superiority of the proposed method.

==> PrefixPages.tex <==
 \chapter*{Dissertation approval}
 \thispagestyle{empty}
 This dissertation entitled {\it \title} by \who~is approved for the degree of \degree.  
 \par
 \vspace{1cm}
 \begin{flushright}
 \begin{tabular}{c}
 \textbf{Examiners}\\
 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
 \\
 \hline
 \\
 \\
 \hline
 \\
 \\
 \textbf{Supervisor}\\
 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
 \\
 \hline
 \\
 \\
 \textbf{Chairman}\\
 ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
 \\
 \hline
 \end{tabular}
 \vspace{2cm}
 \end{flushright}
 \begin{flushleft}
 \begin{tabular}{lc}
 Date:&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
 \cline{2-2}
 \\
 Place:&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
 \cline{2-2}
 \end{tabular}
 \end{flushleft}
%\fullpage{approval}
%\includepdf{approval.pdf} 
\chapter*{Declaration}
\thispagestyle{empty}
I declare that this written submission represents my ideas in my own words and where others ideas or words have been included, I have adequately cited and referenced the original sources. I also declare that I have adhered to all principles of academic honesty and integrity
and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will be cause for disciplinary action by the Institute and can also evoke  penal action from the sources which have thus not been
properly cited or from whom proper permission has not been taken when needed.
\par
\vspace{3cm}

\begin{flushright}
\begin{tabular}{c}
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
\hline
\\
%\textbf{(Roll No: \who)}\\
%\textbf{\roll}
\end{tabular}
\end{flushright}


==> chapter4_Field_Data.tex <==
\chapter{Field Data Performance Analysis}
Bearings only tracking is performed on a field data. The problem is to track a ship using the bearing meausurements obtained from another moving ship. Field data consists of recorded bearing measurements of the target as well as ownship course and speed. All angles are measured cloakwise positive from North. The target ship moves in constant velocity motion of $20$ knots. The observer ship moves in nearly constant speed motion of 12 knots. It undertakes a maneuver in midst of the course. Initial target range is $4000$ $m$ and initial ownship course is $180$ $degrees$. The measurements are obtained at a regular interval of $T=1.28s$. The details of the field data are summarised in Table.\ref{tab:scenarios}. Target estimation is done using extended Kalman filter and particle filter, and their performance is compared.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Field Data}
%    \resizebox{4in}{!}{
    \begin{tabular}{p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}}
    \hline
    S. No & Initial Target Rng (m) & Initial Target Brg (Deg) & Target Crs (Deg) & Target Spd (Knots) & Initial Ownsip Crs (Deg) & Initial Ownship Spd (knots) & Ownship Maneuver Crs (Deg) \\
    \hline
    1     & 4000  & 265   & 121   & 20    & 180   & 12    & 115 \\
    %2     & 4000  & 285   & 140   & 20    & 180   & 12    & 135 \\
    \hline
    \end{tabular}%
% }
  \label{tab:scenarios}%
\end{table}%

\section{Simulation and Results}
The bearings only tracking is done using the technique similar to the one mentioned in \cite{4}. The target state vector is defined to be  
\begin{eqnarray}
\mathbf{x}^{t}_k=
\begin{bmatrix}
x^{t}_k & \dot{x}^{t}_k & y^{t}_k  & \dot{y}^{t}_k
 \end{bmatrix}^T \nonumber
\end{eqnarray}
where $k$ is the time index. The ownship state is also defined as 
\begin{eqnarray}
\mathbf{x}^{o}_k=
\begin{bmatrix}
x^{o}_k & \dot{x}^{o}_k & y^{o}_k  & \dot{y}^{o}_k
 \end{bmatrix}^T \nonumber
\end{eqnarray}. The relative state vector is defined by
\begin{align}
 \mathbf{x}_k & = \mathbf{x}_k^t-\mathbf{x}_k^0\\
& = \begin{bmatrix}
      x &\dot{x} &y &\dot{y}
     \end{bmatrix}^T \nonumber
\end{align}
The ownship initial position is assumed to be at the origin. The initial position of the target is at 4000cos$(265^0)$, 4000sin$(265^0)$. Initial state covariance is assumed to be $P = diag(\begin{matrix}[15&0.2& 15& 0.2]\end{matrix})$. The target has state transition model $\mathbf{F}$ such that:
\begin{eqnarray}
\mathbf{x}_{k} & = & \mathbf{F}(\mathbf{x}_{k-1})+\mathbf{w}_k-\mathbf{U}_{k,k-1} \nonumber
\end{eqnarray}
where $\mathbf{w}_k$ is the process noise with zero mean and covariance $Q_{w}$  and $\mathbf{U}_{k,k-1}$ is the deterministic input accounting for the ownship motion. The matrices $\mathbf{F}$, $Q_{w}$ and $\mathbf{U}_{k,k-1}$ are given by 
\begin{equation}
 \mathbf{F}=\begin{bmatrix}
1&T&0&0\\
0&1&0&0\\
0&0&1&T\\
0&0&0&1\\
\end{bmatrix} \nonumber
\end{equation}
\begin{equation} 
Q_{w} = \begin{bmatrix}
% \sigma_x ,0, \sigma_y ,0 \right)
 \sigma_x^2(T^3)/3    &\sigma_x^2*(T^2)/2   &0 &0\\
        \sigma_x^2(T^2)/2   &\sigma_x^2T               &0 &0\\
        0 &0 &\sigma_y^2(T^3)/3    &\sigma_y^2(T^2)/2 \\
        0 &0 &\sigma_y^2(T^2)/2   &\sigma_y^2T         \\
\end{bmatrix} \nonumber
\end{equation}
\begin{equation}
 \mathbf{U}_{k,k-1} = \begin{bmatrix}
                     \dot{x}_{k}^0-\dot{x}_{k-1}^0 \\0 \\\dot{y}_{k}^0-\dot{y}_{k-1}^0 \\0
                    \end{bmatrix} \nonumber
\end{equation}
where $T$ is the sampling period of the target dynamics and $\sigma_x=\sigma_x=5\times10^{-2}$. $\mathbf{U}_{k,k-1}$ is assumed to be known at every moment. In this simulation, it is calculated from the ownship speed and course available at every instant $k$. The target's bearing $\theta$ at time $k$ is available as the measurement $\theta_{k}$ at time step of $T$ at the ownship. 
\begin{eqnarray}
\theta_{k}=
h(\mathbf{x}_k)+\mathbf{v}_{k}=
\begin{bmatrix}
\tan^{-1}\left(\dfrac{x_{k}}{y_{k}}\right)
\end{bmatrix} \nonumber
\end{eqnarray}                                                      
The error in the bearing is such that $\sigma_\theta=0.1$ radians. Target was at an initial bearing of $265$ degrees and a course of $121$ degrees. 209 measurements were available at sampling rate of $T$ $s$. The estimates of the target states are obtained from the estimates of the relative state vector $\mathbf{x}_k$ by removing the bias due to the ownship, i.e,
\begin{eqnarray}
 \mathbf{x}_k^t=\mathbf{x}_k +\mathbf{x}_k^o \nonumber\\ 
\end{eqnarray}

\subsection{Extended Kalman Filter Estimation}
The true trajectories of the target and their estimates are shown in Fig.\ref{FD_KFS1_xy_plot}. The state estimates of the targets are shown in Fig.\ref{FD_KFS1_state}. The mean square error MSE of the position estimates are shown in Fig.\ref{FD_KFS1_MSE}. The bearing measurement and its estimate are shown in Fig.\ref{FD_KFS1_bearing_meas}.

\begin{figure}[h]
\centering
% \subfloat [IPPF estimate]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/xy_plot}  
} 
% \subfloat [PF estimate]
% {\label{PF_xy_state}\includegraphics[scale=0.5]{IPPF_fig/PF_xy_plot}  
% }\\   
\caption{Target's true $xy$ track and their estimated track is obtained using EKF.}
\label{FD_KFS1_xy_plot}
\end{figure}

\begin{figure}[h]
\centering
% \subfloat [IPPF Target 1 estimate]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/MSE}  
}
\caption{MSE of the position estimates obtained using EKF.}
\label{FD_KFS1_MSE}
\end{figure} 

\begin{figure}[h]
\centering
\subfloat [position $x$ ]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/x_state}  
}\\
\subfloat [position $y$ ]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/y_state}  
}\\
\subfloat [velocity $v_x$]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/vx_state}  
}%
\subfloat [velocity $v_y$]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/vy_state}  
}\\
\caption{Target's true states and their estimates obtained using EKF.}
\label{FD_KFS1_state}
\end{figure} 



\begin{figure}[h]
\centering
% \subfloat [MCJPDAF estimate]
{\includegraphics[scale=0.4]{Field_Data_fig/KF_S1/Bearing}  
} 
% \subfloat [PF estimate]
% {\label{PF_xy_state}\includegraphics[scale=0.5]{IPPF_fig/PF_xy_plot}  
% }\\   
\caption{Targets' true bearing and its estimate using EKF.}
\label{FD_KFS1_bearing_meas}
\end{figure}

\subsection{Particle Filter Estimation}
The number of particles used is $N=1000$. The true trajectories of the target and their estimates are shown in Fig.\ref{FD_PFS1_xy_plot}. The state estimates of the targets are shown in Fig.\ref{FD_PFS1_state}. The mean square error MSE of the position estimates are shown in Fig.\ref{FD_PFS1_MSE}. The bearing measurement and its estimate are shown in Fig.\ref{FD_PFS1_bearing_meas}. The results show that PF has better estimate for the bearing of the target compared to EKF. The state estimates of the target doesn't have much significant difference.

\begin{figure}[h]
\centering
% \subfloat [IPPF estimate]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/xy_plot}  
} 
% \subfloat [PF estimate]
% {\label{PF_xy_state}\includegraphics[scale=0.5]{IPPF_fig/PF_xy_plot}  
% }\\   
\caption{Target's true $xy$ track and their estimated track is obtained using PF.}
\label{FD_PFS1_xy_plot}
\end{figure}

\begin{figure}[h]
\centering
% \subfloat [IPPF Target 1 estimate]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/MSE}  
}
\caption{MSE of the position estimates obtained using PF.}
\label{FD_PFS1_MSE}
\end{figure} 


\begin{figure}[h]
\centering
% \subfloat [MCJPDAF estimate]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/Bearing}  
} 
% \subfloat [PF estimate]
% {\label{PF_xy_state}\includegraphics[scale=0.5]{IPPF_fig/PF_xy_plot}  
% }\\   
\caption{Targets' true bearing and its estimate using PF.}
\label{FD_PFS1_bearing_meas}
\end{figure}

\begin{figure}[h]
\centering
\subfloat [position $x$ ]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/x_state}  
}\\
\subfloat [position $y$ ]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/y_state}  
}\\
\subfloat [velocity $v_x$]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/vx_state}  
}%
\subfloat [velocity $v_y$]
{\includegraphics[scale=0.4]{Field_Data_fig/PF_S1/vy_state}  
}\\
\caption{Target's true states and their estimates obtained using PF.}
\label{FD_PFS1_state}
\end{figure} 







==> declaration.tex <==
\noindent \textbf{\large{Declaration}} \\ 
\noindent I declare that this written submission represents my ideas in my own words and where others ideas or words have been included, I have adequately cited and referenced the original sources. I also declare that I have adhered to all principles of academic honesty and integrity 
and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will be cause for disciplinary action by the Institute and can also evoke  penal action from the sources which have thus not been 
properly cited or from whom proper permission has not been taken when needed.
\vspace{2cm}

\begin{verb}

\hspace{180pt} Signature :\hspace{59pt}  $\hdots$ $\hdots$ $\hdots$ $\hdots$ 

\hspace{180pt} Name of the student :  P. Venkata Srikanth Reddy

\hspace{180pt} Roll No : \hspace{59pt} 08307008
\end{verb}




 


==> hyperlinks.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hyperlinks
\begin{frame}[label=GenerateIndices]{Generating indices from a distribution}

 \begin{figure}[h]
 \centering 
   \includegraphics[scale=0.3]{BootstrapPF_fig/Distribution_sampling_M}
%\caption{Resampling of a set of particles representing a distribution $P(x)$ }

\end{figure}
\end{frame}


\begin{frame}{Generating indices from a distribution}
\begin{table}[H] 
\caption{Method 1: Generating indices from a given distribution} %title of the table 
\centering          % centering table 
\begin{tabular}{l}
  \hline
  \begin{minipage}{4in}
    \vskip 4pt
$[\{j(n)\}_{n=1}^R]=$Generate indices$[\{\rho^{(n)}\}_{n=1}^{N}, R]$
\begin{itemize}
	\item $c(0)=0$ 
	\item FOR $i=1:N$,
	\begin{itemize}
		\item $c(i)=c(i-1)+ \rho^{(i)}$ 		
	\end{itemize}
	\item END FOR
	\item FOR  $n=1:R$,
	\begin{itemize}
	      \item Draw $u_n\sim \mathcal{U} [0,1]$  		
	      \item m=1
	      \item WHILE $(c(m)<u_n)$
	      \begin{itemize}
		    \item$ m=m+1$
	      \end{itemize}
	      \item END WHILE
	      \item Set $j(n)=m$
	\end{itemize}
	\item END FOR
\end{itemize}
   \vskip 4pt
 \end{minipage}
 \\
  \hline
 \end{tabular}
\label{tab:Generate_Dist1} 
\end{table}

\hyperlink{BackGenerateIndices}{back}
\end{frame}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hyperlinks
\begin{frame}[label=AfterPrediction]

 \begin{figure}[H]
 \centering 
   \includegraphics[scale=0.27]{BootstrapPF_fig/BootstrapPF}
\caption{Perform weighted resampling after prediction step and choose likelihood for target $k$ as $g(x)(k)$ \hyperlink{BackAfterPrediction}{back} } 
\label{fig:BootstrapPF}
 \end{figure}
%

\end{frame}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
 \begin{frame}[label=IPPF_Algorithm]{IPPF Algorithm}

 \begin{itemize} 
 	 \item {\color{red}Step:1} Sample particles from importance density using independent partioned sampling.	
	  \begin{itemize}
	   \item For $k=1, 2,..., K_{t}$
		\begin{itemize}
{\normalsize
			\item For $i=1, 2,..., N$ 
			\begin{equation*}
			 \mathbf{x}_t^{(i)}(k) \sim q_{k}(\mathbf{x}_{t}(k)\mid \mathbf{x}_{t-1}^{(i)}(k),z_{t})
			\end{equation*}
			 \begin{equation*}
			      \mathbf{x}_{t}^{(i)}(k) \sim p(\mathbf{x}_{t}(k)\mid \mathbf{x}_{t-1}^{(i)}(k))=\mathcal{N}(a_t^{(i)}(k),Q_{w})
			\end{equation*}
		      \begin{equation*}
			      a_t^{(i)}(k)= F\mathbf{x}_{t-1}^{(i)}(k)
		      \end{equation*}
}
		\end{itemize}
	  \end{itemize}
 \end{itemize}
 \end{frame}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{frame}{IPPF Algorithm}

{\color{red}Step:2} Weighted Resampling
\begin{itemize}
\item {\color{red}Step:2a}Perform Weighted resampling w.r.t likelihood	
	  \begin{itemize}
	   \item For $k=1, 2,..., K_{t}$
		\begin{itemize}%{\normalsize
{\normalsize
		\item For $i=1, 2,..., N$ \\Compute secondary weights using likelihood $p(z_{t}(k)\mid \mathbf{x}_{t}^{i}(k))$ 
			      \begin{equation*}
				    g(\mathbf{x}_{t}^{(i)}(k))=\mathcal{N}(z_t(k);b_t(k),Q_{v:k})
			      \end{equation*}
			      \begin{equation*}
				      b_t(k)=h_k(\mathbf{x}_{t}^{(i)}(k))
			      \end{equation*}
}
	      \end{itemize}
	\end{itemize}
\item {\color{red}Step:2b} For $k=1,2,..K_t$
    \begin{itemize}
    \item For $i=1, 2,..., N$, Normalize the secondary weights
	\begin{equation*}
	    \rho^{(i)}(k)= \frac{g(\mathbf{x}_{t}^{(i)}(k)}{\sum^{N}_{j=1}g(\mathbf{x}_{t}^{(j)}(k)}
	\end{equation*}	
    \end{itemize}
\end{itemize}
\end{frame}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{frame}{IPPF Algorithm}

{\color{red}Step:2} Weighted Resampling
\begin{itemize}
\item {\color{red}Step:2c} For $k=1, 2,..K_t$
    \begin{itemize}
	\item For $i=1, 2,..., N$  
	    \begin{itemize}
{\normalsize
	    \item Sample indices $j_{k}(i)$ from the distribution formed by $\rho^{(n)}(k)$ for $n=1,2,3,...,N$
}
	    \end{itemize}	
    \end{itemize}
% % 
\item {\color{red}Step:2d} For $i=1, 2,..., N$
    \begin{itemize} 
		   
		    \item Set the new particles and weights$$\mathbf{x}_{t}^{(i)} \equiv \{\mathbf{x}_{t}^{(j_{1}(i))}(1),\mathbf{x}_{t}^{(j_{2}(i))}(2),x_{t}^{(j_{3}(i))}(3),.....,\mathbf{x}_{t}^{(j_{K_{t}}(i))}(K_{t})\}$$
		      $$\mathbf{x}_{t}^{(i)} \equiv \{\mathbf{x}_{t}^{(j_{1}(i))}(1),\mathbf{x}_{t}^{(j_{2}(i))}(2)\}$$    
		    $$w_{t-1}^{*(i)} \equiv w_{t-1}^{(j_{1}(i))} \times w_{t-1}^{(j_{2}(i))}$$
    \end{itemize}
\item {\color{red}Step:2e} \item For $i=1, 2,..., N$, normalize weights:
		  $$\tilde{w}^{(i)}_{t-1} =  \dfrac{w^{*(i)}_{t-1}}{\sum^{N}_{j=1}w^{*(j)}_{t-1}}$$
\item {\color{red}Step:2f} Roughen the particles.
 \end{itemize}
\end{frame}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{frame}
 
{\color{red}Step:3} Weight Update
\begin{itemize}
\item For $i=1, 2,..., N$ evaluate the importance weights 
$$ w_{t}^{(i)}=\dfrac{\tilde{w}_{t-1}^{(i)}}{\prod_{k=1}^{K_{t}}\rho^{(j_{k}(i))}(k)} \dfrac{p(z_{t}\rvert  \mathbf{x}_{t}^{(i)}) p(\mathbf{x}_{t}^{(i)}\rvert \mathbf{x}_{t-1}^{(i)})}{q(\mathbf{x}_{t}^{(i)}\mid \mathbf{x}_{t-1}^{(i)},z_{t}) } $$
$$ w_{t}^{(i)}=\frac{\tilde{w}_{t-1}^{(i)} p(z_{t}\rvert \mathbf{x}_{t}^{(i)})}{\prod_{k=1}^{2}\rho^{(j_{k}(i))}(k)} $$
$$p(\mathbf{z}_{t}\rvert \mathbf{x}_{t}^{(i)})=\mathcal{N}(\mathbf{z}_{t};h(\mathbf{x}_{t}^{(i)}),\mathbf{Q_v})$$

\item For $i=1, 2,..., N$, normalize weights:
		  $$w^{(i)}_t =  \dfrac{w^{(i)}_t}{\sum^{N}_{j=1}w^{(j)}_t}$$
\end{itemize}

{\color{red}Step:4} If required resample and roughen particles.
\hyperlink{BackAfterPrediction}{back}
\end{frame}

